Convolutional Pose Machines

Pose Machines provide a sequential prediction framework for learning rich implicit spatial models. In this work we show a systematic design for how convolutional networks can be incorporated into the pose machine framework for learning image features and image-dependent spatial models for the task of pose estimation. The contribution of this paper is to implicitly model long-range dependencies between variables in structured prediction tasks such as articulated pose estimation. We achieve this by designing a sequential architecture composed of convolutional networks that directly operate on belief maps from previous stages, producing increasingly refined estimates for part locations, without the need for explicit graphical model-style inference. Our approach addresses the characteristic difficulty of vanishing gradients during training by providing a natural learning objective function that enforces intermediate supervision, thereby replenishing back-propagated gradients and conditioning the learning procedure. We demonstrate state-of-the-art performance and outperform competing methods on standard benchmarks including the MPII, LSP, and FLIC datasets.

==> sections/intro_2.tex <==
%!TEX root = ../ICCV2015DeepPose.tex
In this work, we introduce \emph{Convolutional Pose Machines} for the task of articulated pose estimation. Convolutional pose machines inherit the benefits of the recently proposed \posemachine\cite{Ramakrishna2014posemachines} architecture---the implicit learning of long-range dependencies between image, multi-scale and multi-part cues--- and combine them with the advantages afforded by convolutional architectures:the ability to directly learn feature representations for both image and spatial context directly from data; a differentiable architecture that allows for all stages to be trained jointly with backpropagation and the ability to efficiently handle large amounts of training data.

Convolutional pose machines consist of a sequence of prediction networks trained to predict confidences for location of each part, improving their predictions in each stage of the sequence (Figure \ref{fig:teaser}).  When convolutional networks are composed in such a way, it results in an overall network with many layers that is at risk of of the problem of \emph{vanishing gradients}\cite{bradley2010learning,glorot2010understanding} during learning. This can occur because backpropagated gradients diminish in strength as they are propagated through the many layers of the network. Convolutional Pose Machines suggest a systematic framework that replenishes gradients by enforcing intermediate supervision periodically through the network.

The design of the network in each stage of our sequential prediction framework is driven by the goal of achieving a large receptive field on both the image and the output of the preceding stage. We find, through experiment, that large receptive fields are crucial for learning long range spatial relationships and result in improved accuracy. Large receptive fields can be achieved by several designs, each with trade-offs in either precision of localization, increase in parameters or increase in depth. We discuss the trade-offs associated with the design and arrive at a network that achieves a large receptive field allowing for the encoding of long range dependencies. The main contribution of this paper is a systematic approach to composing convolutional networks with large receptive fields for pose estimation tasks, which addresses the vanishing gradients problem by enforcing intermediate supervision.We demonstrate state-of-the-art performance of our system on standard benchmarks and outperform competing methods.




==> sections/intro_3.tex <==
%!TEX root = ../ICCV2015DeepPose.tex
\section{Introduction}

%Improvements in pose estimation of articulated objects have been mainly due to two reasons. The first is due to advances in developing feature representations which make the maximal use of image evidence \cite{jain2014learning,pishchulin13iccv} and the second is due to methods that are capable of sophisticated spatial modeling \cite{tompson2014joint,Ramakrishna2014posemachines,pishchulin2013poselet}.
%Recent work \cite{Ramakrishna2014posemachines} introduced the modular \emph{\posemachine} framework which allows for the implicit learning  of complicated dependencies between part appearance and location, but relies on classical hand-crafted features for representing both image and spatial context information. In this work, we combine the rich spatial modeling afforded by the \posemachine~framework with recent advances in deep convolutional architectures to design a \emph{Convolutional Pose Machine}. Convolutional Pose Machines learn the image and spatial context representations directly from data, and the differentiability of the network allows joint training of all stages and levels through back propagation
We introduce \emph{Convolutional Pose Machines} for the task of articulated pose estimation. Convolutional pose machines inherit the benefits of the recently proposed \emph{\posemachine} \cite{Ramakrishna2014posemachines} architecture---the implicit learning of long-range dependencies between image, multi-scale and multi-part cues, tight integration between learning and inference, a modular sequential design---and combine them with the advantages afforded by convolutional architectures: the ability to learn feature representations for both image and spatial context directly from data; a differentiable architecture that allows for all stages to be trained jointly with backpropagation; and the ability to efficiently handle large training datasets.

Convolutional pose machines consist of a sequence of prediction networks trained to predict confidences for the locations of each part, improving their predictions in each stage of the sequence (Figure \ref{fig:teaser}).  When convolutional networks are composed in such a way, it results in an overall network with many layers that is at risk of the problem of \emph{vanishing gradients} \cite{hochreiter2001gradient,bradley2010learning,glorot2010understanding,bengio1994learning} during learning. This problem can occur because backpropagated gradients diminish in strength as they are propagated through the many layers of the network.  While there exists recent work which shows that supervising very deep networks at intermediate layers aids in learning \cite{lee2014deeply,szegedy2014going}, they have mostly been restricted to simpler classification problems. In this work, we show how for a \emph{structured prediction} problem such as pose estimation, Convolutional Pose Machines naturally suggest a systematic framework that replenishes gradients by enforcing intermediate supervision periodically through the network.
\begin{figure}[t!]
    \centering
    \includegraphics[width=1\columnwidth]{figures/teaser_cr-crop.pdf}
    \caption{A \textbf{Convolutional Pose Machine} consists of a sequence of predictors trained to make a dense predictions at each image location. Here we show the increasingly refined estimates for the location of the \emph{right wrist} in each stage of the sequence.}
    \label{fig:teaser}
\end{figure}

The design of the network in each stage of our sequential prediction framework is motivated by the goal of achieving a large receptive field on both the image and the output predictions of the preceding stage. We find, through experiment, that large receptive fields are crucial for learning long range spatial relationships and result in improved accuracy. Large receptive fields could be achieved by different designs: increasing pooling; increasing the number of layers; or increasing the kernel size of each convolutional filter. Each of these design choices come with trade-offs in either precision of localization, increase in network depth, or increase in parameters.  We discuss the design of a convolutional architecture with intermediate supervision that achieves a large receptive field allowing for the encoding of long range spatial dependencies.

Our main contributions are (a) a sequential convolutional architecture that directly learns both image and image-dependent spatial context from data and 
(b) 
%building on the pose machine framework, we provide 
a systematic approach to composing convolutional networks with large receptive fields for pose estimation tasks without the need for any graphical model style inference. We achieve state-of-the-art results on standard benchmarks, and analyze the effects of using an architecture with intermediate supervision, providing further evidence that networks with large depths can be effectively learned via intermediate supervision.
%Each stage in the sequential prediction framework uses as features information from both local image evidence as well as spatial context information from confidence map predictions of the preceding stage. In order to model long range spatial relationships we require networks with large receptive fields. Large receptive fields can be achieved either by pooling, at the expense of precision, or by increasing the number of layers, increasing the susceptibility to vanishing gradients. The contribution of this paper is a systematic approach to composing convolutional networks with large receptive fields for pose estimation tasks, which elegantly addresses the vanishing gradients problem by enforcing intermediate supervision. We demonstrate state-of-the-art performance of our system on standard benchmarks and outperform competing methods. We make the following technical contributions:


%%%%%

% Recent work \cite{Ramakrishna2014posemachines} introduced the modular \emph{\posemachine} framework which allows for the implicit learning of complicated dependencies between part appearance and location. However, the model relies on classical hand-crafted features for representing both image and spatial context information. In this work, we combine the rich spatial modeling afforded by the \posemachine~framework with recent advances in deep convolutional architectures for supervised feature learning to directly learn, without manual design, feature representations for both image and spatial context information.

% The pose machine architecture consists of a sequence of predictors trained to predict confidences for locations of the parts, improving their predictions in each stage (Figure \ref{fig:teaser}). When convolutional networks are composed in the framework of a pose machine, the resulting deepening of the network can be susceptible to the problem of \emph{vanishing gradients}. Networks with a large number of layers can be challenging to train as the backpropagated gradients diminish in strength as they are propagated through the network \cite{bradley2010learning,glorot2010understanding}. We show how the sequential prediction framework of a \posemachine~provides a natural learning objective that enforces intermediate supervision periodically through the network thus replenishing backpropagated gradients at each stage.
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=1\columnwidth]{figures/teaser_half}
%     \caption{A \textbf{Convolutional Pose Machine} consists of a sequence of predictors trained to make a dense predictions at each image location. Here we show the increasingly refined estimates for the location of the \emph{right wrist} in each stage of the sequence.}
%     \label{fig:teaser}
% \end{figure}

% Each stage in the sequential prediction framework uses as features information from both local image evidence as well as spatial contextual information from predictions of the preceding stage of the sequence. To model the spatial relationships between body parts, large receptive fields are needed because long range spatial relationships are informative. Large receptive fields can be achieved either by pooling, at the expense of precision, or by increasing the number of layers, increasing the susceptibility to vanishing gradients. We demonstrate state-of-the-art performance of our system on standard benchmarks and outperform all competing methods on the LSP and FLIC benchmarks. Our contributions are:
% \begin{itemize}
% \setlength{\itemsep}{1pt}
% \setlength{\parskip}{1pt}
% \setlength{\parsep}{1pt}
% 	\item[---] A systematic approach to composing convolutional networks with large receptive fields for pose estimation tasks, which  addresses the vanishing gradients problem by enforcing intermediate supervision to replenish backpropagated gradients.

% 	\item[---] We show how a \emph{Convolutional Pose Machine} with many layers can be trained by using a learning objective that enforces local supervision after every stage.
% \end{itemize}

